Towards Practical Requirement Analysis and Verification: A Case Study on Software IP Components in Aerospace Embedded Systems

IP-based software design is a crucial research field that aims to improve efficiency and reliability by reusing complex software components known as intellectual property (IP) components. To ensure the reusability of these components, particularly in security-sensitive software systems, it is necessary to analyze the requirements and perform formal verification for each IP component. However, converting the requirements of IP components from natural language descriptions to temporal logic and subsequently conducting formal verification demands domain expertise and non-trivial manpower. This paper presents a case study on software IP components derived from aerospace embedded systems, with the objective of automating the requirement analysis and verification process. The study begins by employing Large Language Models to convert unstructured natural language into formal specifications. Subsequently, three distinct verification techniques are employed to ascertain whether the source code meets the extracted temporal logic properties. By doing so, five real-world IP components from the China Academy of Space Technology (CAST) have been successfully verified.

==> Listing/Code1.tex <==
// Interface.h
extern void Fg333saCheckFun(void *p);

typedef struct Fg333saCheck {
    ...
	const uint08 *buffer;
	uint32 rdLen;
	uint32 frm;
	uint32 bComSuc;
    ...
	int32 cntLenRd;
	int32 cntHead;
	int32 cntCheck;
	int32 cntUpdata;
	int32 totalLenRd;
	int32 totalHead;
	int32 totalCheck;
	int32 totalUpdata;
    ...
}Fg333saCheck;

==> Listing/Listing1.tex <==
\definecolor{stubbg}{HTML}{FCF3D5}

\lstinputlisting[
    language=c,
    %basicstyle=\linespread{1.0}\tiny,
    morekeywords={var},
    aboveskip=0pt,
    belowskip=10pt,
    float=tb,
    caption=Partial Interface Implementation Sample,
    label={listing:case-study-interface},
    escapechar=|,
    numbers=left
]{Listing/Code1.tex}
